CIARD: Cyclic Iterative Adversarial Robustness Distillation

Adversarial robustness distillation (ARD) aims to transfer both performance and robustness from teacher model to lightweight student model, enabling resilient performance on resource-constrained scenarios. Though existing ARD approaches enhance student model's robustness, the inevitable by-product leads to the degraded performance on clean examples. We summarize the causes of this problem inherent in existing methods with dual-teacher framework as: 1. The divergent optimization objectives of dual-teacher models, i.e., the clean and robust teachers, impede effective knowledge transfer to the student model, and 2. The iteratively generated adversarial examples during training lead to performance deterioration of the robust teacher model. To address these challenges, we propose a novel Cyclic Iterative ARD (CIARD) method with two key innovations: a. A multi-teacher framework with contrastive push-loss alignment to resolve conflicts in dual-teacher optimization objectives, and b. Continuous adversarial retraining to maintain dynamic teacher robustness against performance degradation from the varying adversarial examples. Extensive experiments on CIFAR-10, CIFAR-100, and Tiny-ImageNet demonstrate that CIARD achieves remarkable performance with an average 3.53 improvement in adversarial defense rates across various attack scenarios and a 5.87 increase in clean sample accuracy, establishing a new benchmark for balancing model robustness and generalization. Our code is available at https://github.com/eminentgu/CIARD

==> _constants.tex <==
\def\paperID{3556}
\def\confName{ICCV}
\def\confYear{2025}

\def\paperTitle{Paper Title}

\def\authorBlock{
    Author 1\thanks{Equal contribution} \qquad
    Author 2\footnotemark[1] \qquad
    Author 3 \\
    Institute \\
    {\tt\small \{email, addresses\}@inst.edu}
}

% Compilation vars
\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}


==> _macros.tex <==
%% PACKAGES (also see cvpr_header.tex)

% \usepackage{graphicx}	
% \usepackage{amsmath}	
% \usepackage{amssymb}	
% \usepackage{booktabs}
\usepackage{times}
\usepackage{microtype}
\usepackage{epsfig}
\usepackage{caption}
\usepackage{float}
\usepackage{placeins}
\usepackage{color, colortbl}
\usepackage{stfloats}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xstring}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{url}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage[hang,flushmargin]{footmisc}

% Unfortunately, this package interferes with arxiv's stamp
\ifcamera \usepackage[accsupp]{axessibility} \fi

%% MACROS

% \newcommand{\authorname}[1]{{\textcolor{blue}{[Author: #1]}}}
% ...

% \newcommand{\commandname}{string\xspace}
% \definecolor{colorname}{rgb}{0.92,0.49,0.19}

% General

\newcommand{\nbf}[1]{{\noindent \textbf{#1.}}}

\newcommand{\supp}{supplemental material\xspace}
\ifarxiv \renewcommand{\supp}{appendix\xspace} \fi

\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}

% Reviewer commands (1 to 5), e.g. \R{1}, \R{2}
\newcommand{\R}[1]{{%
    \textbf{%
        \ifstrequal{#1}{1}{\textcolor{red}{R#1}}{%
        \ifstrequal{#1}{2}{\textcolor{blue}{R#1}}{%
        \ifstrequal{#1}{3}{\textcolor{magenta}{R#1}}{%
        \ifstrequal{#1}{4}{\textcolor{teal}{R#1}}{%
                           \textcolor{cyan}{R#1}%
        }}}}%
    }%
}}


\usepackage{natbib}
% \setcopyright{none}
% \citestyle{acmauthoryear}
\usepackage{algpseudocode}
\usepackage{url}
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{ulem} 
\usepackage{multicol}
\usepackage{indentfirst}
\usepackage{enumitem}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{cancel}
\usepackage{booktabs}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{ulem}
\usepackage{makecell}
\usepackage{booktabs}       % 专业表格样式
\usepackage{siunitx}        % 数字对齐
\usepackage{xcolor}         % 颜色支持
% \usepackage[hidelinks]{hyperref}
% \usepackage{hyperref} 
% \hypersetup{
%     colorlinks=true,
%     linkcolor=blue,   % 设置章节和引用的链接为蓝色
%     urlcolor=blue,    % 设置URL链接为蓝色
%     citecolor=blue    % 设置文献引用为蓝色
% }
\usepackage{setspace}
\newlength{\commentlen}
\usepackage{amsmath}
% Add packages here
% \usepackage[utf8]{inputenc}
% Our math definitions
\newcommand{\unlearn}[2]{{#1 \rightarrow #2}}
\newcommand{\point}{z}
\newcommand{\pert}{\tilde{z}}
\newcommand{\points}{Z}
\newcommand{\perts}{\tilde{Z}}
\newcommand{\loss}{\ell}
\newcommand{\gradlossPoint}{\nabla_{\model}\loss(\point, \optmodel)}
\newcommand{\gradlossPert}{\nabla_{\model}\loss(\pert, \optmodel)}
\newcommand{\bigloss}{L}
\newcommand{\optmodel}{\theta^*}
\newcommand{\model}{\theta}
\newcommand{\Model}{\Theta}
\newcommand{\feat}{f}
\newcommand{\feats}{F}
\newcommand{\val}{v}
\newcommand{\vals}{V}
\newcommand{\lipschitz}{Lipschitz continuity\xspace}

\let\oldparagraph\paragraph
\renewcommand{\paragraph}[1]{\vspace{2pt}\noindent\textbf{#1.}}
\newcommand{\quasipara}[1]{\vspace{1pt}\noindent\emph{#1.}}
\renewcommand{\algorithmicrequire}{ \textbf{Input:}}

% Reference commands
\newcommand{\tab}[1]{\cref{#1}}
\newcommand{\fig}[1]{\cref{#1}}
\newcommand{\sect}[1]{\cref{#1}}
\newcommand{\appdx}[1]{\cref{#1}}

\SetKwInput{KwInput}{Input}           % input for algorithm package
\SetKwInput{KwOutput}{Output}         % output for algortihm package
\setlength{\belowcaptionskip}{-1em}

==> cvpr_header.tex <==
\ifreview \usepackage[review]{cvpr} \fi
\ifarxiv \usepackage[pagenumbers]{cvpr} \fi
\ifrebuttal \usepackage[rebuttal]{cvpr} \fi
\ifcamera \usepackage{cvpr} \fi

\input{_macros}  % Add packages to _macros.tex

%% For cross-referencing labels between documents
\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,allcolors=cvprblue]{hyperref}
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}

\ifarxiv \crefname{appendix}{App.}{Apps.}
\else \crefname{appendix}{Suppl.}{Suppls.} \fi

\frenchspacing


==> sec/5_experiment_results.tex <==
% \section{Experiment Results}
% \label{sec:experiment_results}

% \subsection{Effectiveness of CIARD}
% Adversarial attacks can be categorized into two types based on the threat model: white-box and black-box attacks. In a white-box setting, the attacker has complete access to the deep learning model, including its architecture and parameters. In contrast, a black-box setup only allows the attacker to access  the model's output.

% \noindent\textbf{White-box Robustness of Student Models.}
% \label{Section:White-Box_Robustness}
% To evaluate robustness against white-box attacks, we tested the student models ResNet-18 and MobileNet-V2 on CIFAR-10 and CIFAR-100 using four attack methods: FGSM, PGD$_{\textup{SAT}}$, PGD$_{\textup{TRADES}}$, and $\textup{CW}_{\infty}$. The experimental results are presented in Tables~\ref{tab_eval_White_cifar10_cifar100_ResNet18} and ~\ref{tab_eval_White_cifar10_cifar100_MobileNet-V2}. Notably, compared to other benchmark methods, CIARD requires only 240 training rounds to achieve a better trade-off between model robustness and classification accuracy.

% As shown in Tables~\ref{tab_eval_White_cifar10_cifar100_ResNet18} and ~\ref{tab_eval_White_cifar10_cifar100_MobileNet-V2}, CIARD's W-Robust accuracy on CIFAR-10 and CIFAR-100 outperforms other ARD methods in most cases. For ResNet-18, weighted robustness improves by 3.41\% and 4.1\%, respectively. Additionally, the cyclic iteration mechanism in CIARD improves the student model's classification accuracy, reaching 89.97\% and 65.99\% on CIFAR-10 and CIFAR-100, respectively. For MobileNet-V2, the results are similar, particularly under FGSM attacks, where weighted robustness improves by 5.63\% and 3.18\% compared to the best benchmark method.



% \begin{table*}[htbp]
% \centering
% \caption{White-box Adversarial Robustness of ResNet-18 on CIFAR-10 and CIFAR-100 Datasets. The best results are \textbf{bolded}, and the second best results are \uline{underlined}.}
% \label{tab_eval_White_cifar10_cifar100_ResNet18}
% \setlength{\tabcolsep}{1.8pt}  % 调整列间距
% \begin{tabular}{l|l|c||cc|cc|cc|cc}
% \toprule
% \multirow{2}{*}{Dataset} & \multirow{2}{*}{Defense} & \multicolumn{3}{c|}{FGSM~\cite{goodfellow2014explaining}} & \multicolumn{2}{c|}{PGD$_\text{sat}$~\cite{madry2017towards}} & \multicolumn{2}{c|}{PGD$_\text{trades}$~\cite{zhang2019theoretically}} & \multicolumn{2}{c}{CW$_{\infty}$~\cite{carlini2017towards}} \\
% \cline{3-11}
%  &  & Clean & Robust & W-Robust & Robust & W-Robust & Robust & W-Robust & Robust & W-Robust \\
% \midrule
% \multirow{11}{*}{CIFAR-10} & Natural & 94.57  & 18.60  & 56.59   & 0   & 47.29   & 0  & 47.29 & 0  & 47.29 \\
% & SAT~\cite{madry2017towards}        & 84.20  & 55.59  & 69.90   & 45.95  & 65.08 & 48.12  & 66.16 & 45.97 & 65.09 \\
% & TRADES~\cite{zhang2019theoretically} & 83.00 & 58.35 & 70.68 & 52.35  & 67.68  & 53.83  & 68.42 & 50.23  & 66.62 \\
% & ARD~\cite{goldblum2020adversarially} & 84.11 & 58.40 & 71.26 & 50.93  & 67.52  & 52.96 & 68.54  & 50.15  & 67.13 \\
% & RSLAD~\cite{zi2021revisiting}      & 83.99  & 60.41  & 72.20  & \uline{53.94}  & 68.97  & \uline{55.73}  & 69.86    & \textbf{52.67}  & 68.33 \\
% & SCORE~\cite{pang2022robustness}    & 84.43  & 59.84  & 72.14  & 53.72  & 69.08 & 55.21  & 69.82 & 50.46  & 67.45 \\
% & Fair-ARD~\cite{yue2024revisiting}  & 83.41  & 58.91  & 71.16  & 52.00  & 67.71 & 53.77  & 68.59 & 51.07  & 67.24 \\
% & ABSLD~\cite{zhao2023improving}     & 83.21  & 60.22  & 71.72  & \textbf{54.63}  & 68.92 & \textbf{56.10}  & 69.66   & \uline{52.04}  & 67.63 \\
% & MTARD~\cite{zhao2022enhanced}     & 87.36 & 61.20  & 74.28  & 50.73  & 69.05  & 53.60  & 70.48  & 48.57  & 67.97 \\
% & B-MTARD~\cite{zhao2024mitigating}    & \uline{88.20}  & \uline{61.42}  & \uline{74.81}  & 51.68  & \uline{69.94}  & 54.40  & \uline{71.30}  & 49.88  & \uline{69.04} \\
% & CIARD      & \textbf{89.69}  & \textbf{61.83}  & \textbf{75.76}  & 51.45  & \textbf{70.57} & 54.46  & \textbf{72.08} & 50.19  & \textbf{69.94} \\
% \midrule
% \multirow{11}{*}{CIFAR-100} & Natural    & 75.18  & 7.96  & 41.57  & 0  & 37.59  & 0  & 37.59  & 0 & 37.59  \\
% & SAT~\cite{madry2017towards}         & 56.16  & 25.88  & 41.02  & 21.18 & 38.67  & 22.02  & 39.09  & 20.90  & 38.53 \\
% & TRADES~\cite{zhang2019theoretically} & 57.75  & 31.36  & 44.56  & 28.05  & 42.90  & 28.88  & 43.32  & 24.19  & 40.97 \\
% & ARD~\cite{goldblum2020adversarially} & 60.11  & 33.61  & 46.86  & 29.40  & 44.76  & 30.51  & 45.31  & 27.56  & 43.84 \\
% & RSLAD~\cite{zi2021revisiting}       & 58.25  & 34.73  & 46.49  & 31.19  & 44.72  & 32.05  & 45.15  & 28.21  & 43.23 \\
% & SCORE~\cite{pang2022robustness}     & 56.40  & 32.94  & 44.67  & 30.27  & 43.34  & 30.56  & 43.48  & 26.30  & 41.35 \\
% & Fair-ARD~\cite{yue2024revisiting}   & 57.81  & 34.39  & 46.10  & 30.64  & 44.23  & 31.05  & 44.66  & 27.84  & 42.83 \\
% & ABSLD~\cite{zhao2023improving}      & 56.77  & 34.94  & 45.86  & 32.41  & 44.59  & 32.99  & 44.88  & 29.99  & 41.88 \\
% & MTARD~\cite{zhao2022enhanced}       & 64.30  & 31.49  & 47.90  & 24.95  & 44.63  & 26.75  & 45.53  & 23.42  & 43.86 \\
% & B-MTARD~\cite{zhao2024mitigating}   & \uline{65.08}  & \uline{34.21}  & \uline{49.65}  & \uline{28.50}  & \uline{46.79}  & \uline{29.94}  & \uline{47.51}  & \uline{25.45}  & \uline{45.27} \\
% & CIARD      & \textbf{65.99}  & \textbf{38.01}  & \textbf{52.00}  & \textbf{33.15}  & \textbf{49.08} & \textbf{34.02}  & \textbf{49.51} & \textbf{30.54}  & \textbf{47.27} \\
% \bottomrule
% \end{tabular}
% \end{table*}





% % \begin{table}[htbp]\small
% % \centering
% % \begin{center}
% % \caption{White-box Adversarial Robustness of ResNet-18 on CIFAR-10 and CIFAR-100 Datasets. The best results are \textbf{bolded}, and the second best results are \uline{underlined}.}
% % \label{tab_eval_White_cifar10_cifar100_ResNet18}
% % \vspace{-0.1in}
% % \setlength{\tabcolsep}{0.1mm}{
% % \begin{tabular}{c|c|ccc|ccc}
% % \toprule
% % \multirow{2}{*}{Attack} & \multirow{2}{*}{Defense} & \multicolumn{3}{c|}{CIFAR-10} & \multicolumn{3}{c}{CIFAR-100} \\
% %  &  & Clean & Robust & W-Robust & Clean & Robust & W-Robust \\
% % \midrule
% % \multirow{11}{*}{FGSM} 
% % & Natural    & 94.57  & 18.60  & 56.59                      & 75.18  & 7.96   & 41.57 \\
% % & SAT        & 84.20  & 55.59  & 69.90                      & 56.16  & 25.88  & 41.02 \\
% % & TRADES     & 83.00  & 58.35  & 70.68                      & 57.75  & 31.36  & 44.56 \\
% % & ARD        & 84.11  & 58.40  & 71.26                      & 60.11  & 33.61  & 46.86 \\
% % & RSLAD      & 83.99  & 60.41  & 72.20                      & 58.25  & 34.73  & 46.49 \\
% % & SCORE      & 84.43  & 59.84  & 72.14                      & 58.25  & 34.73  & 46.49 \\
% % & Fair-ARD   & 83.41  & 58.91  & 71.16                      & 58.25  & 34.73  & 46.49 \\
% % & ABSLD      & 83.21  & 60.22  & 71.72                      & 58.25  & 34.73  & 46.49 \\
% % & MTARD      & 87.36  & 61.20  & 74.28                      & 64.30  & 31.49  & \cellcolor{gray!40}47.90  \\
% % & B-MTARD    & \uline{88.20}  & \uline{61.42}  & \uline{74.81}   & 64.30  & 31.49  & \cellcolor{gray!40}47.90  \\
% % & CIARD      & \textbf{89.69}  & \textbf{61.83}  & \textbf{75.76}             & 65.99  & 38.01  & \textbf{52.00} \\
% % \cmidrule{1-8}
% % \multirow{11}{*}{PGD$_\text{sat}$} 
% % & Natural    & 94.57  & 0      & 47.29                      & 75.18  & 7.96   & 41.57 \\
% % & SAT        & 84.20  & 45.95  & 65.08                      & 56.16  & 25.88  & 41.02 \\
% % & TRADES     & 83.00  & 52.35  & 67.68                      & 57.75  & 31.36  & 44.56 \\
% % & ARD        & 84.11  & 50.93  & 67.52                      & 60.11  & 33.61  & 46.86 \\
% % & RSLAD      & 83.99  & \uline{53.94}  & 68.97                      & 58.25  & 34.73  & 46.49 \\
% % & SCORE      & 84.43  & 53.72  & 69.08                      & 58.25  & 34.73  & 46.49 \\
% % & Fair-ARD   & 83.41  & 52.00  & 67.71                      & 58.25  & 34.73  & 46.49 \\
% % & ABSLD      & 83.21  & \textbf{54.63}  & 68.92                      & 58.25  & 34.73  & 46.49 \\
% % & MTARD      & 87.36  & 50.73  & 69.05                      & 64.30  & 31.49  & 47.90  \\
% % & B-MTARD    & \uline{88.20}  & 51.68  & \uline{69.94}              & 64.30  & 31.49  & 47.90  \\
% % & CIARD      & \textbf{89.69} & 51.45  & \textbf{70.57}    & 65.99  & 38.01  & \textbf{52.00} \\
% % \cmidrule{1-8}
% % \multirow{11}{*}{PGD$_\text{trades}$} 
% % & Natural    & 94.57  & 0      & 47.29                      & 75.18  & 7.96   & 41.57 \\
% % & SAT        & 84.20  & 48.12  & 66.16                      & 56.16  & 25.88  & 41.02 \\
% % & TRADES     & 83.00  & 53.83  & 68.42                      & 57.75  & 31.36  & 44.56 \\
% % & ARD        & 84.11  & 52.96  & 68.54                      & 60.11  & 33.61  & 46.86 \\
% % & RSLAD      & 83.99  & \uline{55.73}  & 69.86                      & 58.25  & 34.73  & 46.49 \\
% % & SCORE      & 84.43  & 55.21  & 69.82                      & 58.25  & 34.73  & 46.49 \\
% % & Fair-ARD   & 83.41  & 53.77  & 68.59                      & 58.25  & 34.73  & 46.49 \\
% % & ABSLD      & 83.21  & \textbf{56.10}  & 69.66                      & 58.25  & 34.73  & 46.49 \\
% % & MTARD      & 87.36  & 53.60  & 70.48                      & 64.30  & 31.49  & 47.90  \\
% % & B-MTARD    & \uline{88.20}  & 54.40  & \uline{71.30}              & 64.30  & 31.49  & 47.90  \\
% % & CIARD      & \textbf{89.69} & 54.46  & \textbf{72.08}    & 65.99  & 38.01  & \textbf{52.00} \\
% % \cmidrule{1-8}
% % \multirow{11}{*}{CW$_{\infty}$} 
% % & Natural    & 94.57  & 0      & 47.29                      & 75.18  & 7.96   & 41.57 \\
% % & SAT        & 84.20  & 45.97  & 65.09                      & 56.16  & 25.88  & 41.02 \\
% % & TRADES     & 83.00  & 50.23  & 66.62                      & 57.75  & 31.36  & 44.56 \\
% % & ARD        & 84.11  & 50.15  & 67.13                      & 60.11  & 33.61  & 46.86 \\
% % & RSLAD      & 83.99  & \textbf{52.67}  & 68.33                      & 58.25  & 34.73  & 46.49 \\
% % & SCORE      & 84.43  & 50.46  & 67.45                      & 58.25  & 34.73  & 46.49 \\
% % & Fair-ARD   & 83.41  & 51.07  & 67.24                      & 58.25  & 34.73  & 46.49 \\
% % & ABSLD      & 83.21  & \uline{52.04}  & 67.63                     & 58.25  & 34.73  & 46.49 \\
% % & MTARD      & 87.36  & 48.57  & 67.97                      & 64.30  & 31.49  & 47.90  \\
% % & B-MTARD    & \uline{88.20}  & 49.88  & \uline{69.04}              & 64.30  & 31.49  & 47.90  \\
% % & CIARD      & \textbf{89.69} & 50.19  & \textbf{69.94}    & 65.99  & 38.01  & \textbf{52.00} \\
% % \bottomrule
% % \end{tabular}
% % }
% % \vspace{-0.075in}
% % \end{center}
% % \end{table}

% \begin{table*}[htbp]
% \centering
% \caption{White-box Adversarial Robustness of MobileNet-V2 on CIFAR-10 and CIFAR-100 Datasets.}
% \label{tab_eval_White_cifar10_cifar100_MobileNet-V2}
% \setlength{\tabcolsep}{1.8pt}  % 调整列间距
% \begin{tabular}{l|l|c||cc|cc|cc|cc}
% \toprule
% \multirow{2}{*}{Dataset} & \multirow{2}{*}{Defense} & \multicolumn{3}{c|}{FGSM~\cite{goodfellow2014explaining}} & \multicolumn{2}{c|}{PGD$_\text{sat}$~\cite{madry2017towards}} & \multicolumn{2}{c|}{PGD$_\text{trades}$~\cite{zhang2019theoretically}} & \multicolumn{2}{c}{CW$_{\infty}$~\cite{carlini2017towards}} \\
% \cline{3-11}
%  &  & Clean & Robust & W-Robust & Robust & W-Robust & Robust & W-Robust & Robust & W-Robust \\
% \midrule
% \multirow{11}{*}{CIFAR-10} & Natural & 93.35  & 12.22  & 52.79  & 0 & 46.68   & 0  & 46.68  & 0  & 46.68 \\
% & SAT~\cite{madry2017towards}        & 83.87  & 55.89  & 69.88  & 46.84  & 65.36 & 49.14  & 66.51 & 46.62 & 65.25 \\
% & TRADES~\cite{zhang2019theoretically} & 77.95  &53.75 &65.85 &49.06 &63.51 &50.27 &64.11 &46.06 &62.01 \\
% & ARD~\cite{goldblum2020adversarially} & 83.43 &57.03 &70.23 &49.50 &66.47 &51.70 &67.57 &48.96 &66.20 \\
% & RSLAD~\cite{zi2021revisiting}      & 83.20  &59.47 &71.34 &53.25 &68.23 &54.76 &68.98 &51.78 &67.49\\
% & SCORE~\cite{pang2022robustness}    & 82.32  &58.43 &70.38 &53.42 &67.87 &54.46 &68.39 &49.18 &65.75 \\
% & Fair-ARD~\cite{yue2024revisiting}  & 82.65  &56.37 &69.51 &50.50 &66.58 &52.12 &67.39 &51.07 &66.86 \\
% & ABSLD~\cite{zhao2023improving}     & 82.50  &58.47 &70.49 &52.98 &67.74 &54.49 &68.50 &50.20 &66.35 \\
% & MTARD~\cite{zhao2022enhanced}      & 89.26  &57.84 &73.55 &44.16 &66.71 &47.99 &68.63 &43.42 &66.34 \\
% & B-MTARD~\cite{zhao2024mitigating}  & 89.09  &58.79 &73.94 &47.56 &68.33 &50.44 &69.77 &46.81 &67.95 \\
% & CIARD      & \textbf{89.69}  & \textbf{61.83}  & \textbf{75.76}  & 51.45  & \textbf{70.57} & 54.46  & \textbf{72.08} & 50.19  & \textbf{69.94} \\
% \midrule
% \multirow{11}{*}{CIFAR-100} & Natural  &74.86 &5.94 &40.40 &0 &37.43 &0 &37.43 &0 &37.43 \\
% & SAT~\cite{madry2017towards}          &59.19 &30.88 &45.04 &25.64 &42.42 &26.96 &43.08 &25.01 &42.10 \\
% & TRADES~\cite{zhang2019theoretically} &55.41 &30.28 &42.85 &23.33 &39.37 &28.42 &41.92 &27.72 &41.57 \\
% & ARD~\cite{goldblum2020adversarially} &60.45 &32.77 &46.61 &28.69 &44.57 &29.63 &45.04 &26.55 &43.50\\
% & RSLAD~\cite{zi2021revisiting}        &59.01 &33.88 &46.45 &30.19 &44.60 &31.19 &45.10 &27.98 &43.50\\
% & SCORE~\cite{pang2022robustness}      &49.38 &29.28 &39.33 &27.03 &38.21 &27.53 &38.46 &23.29 &36.34\\
% & Fair-ARD~\cite{yue2024revisiting}    &59.18 &34.07 &46.63 &30.15 &44.67 &31.26 &45.22 &27.55 &43.37 \\
% & ABSLD~\cite{zhao2023improving}       &56.67 &33.85 &45.26 &31.28 &43.98 &31.90 &44.29 &26.40 &41.54\\
% & MTARD~\cite{zhao2022enhanced}        &67.01 &32.42 &49.72 &25.14 &46.08 &27.10 &47.06 &24.14 &45.58\\
% & B-MTARD~\cite{zhao2024mitigating}    &66.13 &34.36 &50.25 &28.47 &47.30 &29.82 &47.98 &26.50 &46.32\\
% & CIARD      & \textbf{65.99}  & \textbf{38.01}  & \textbf{52.00}  & \textbf{33.15}  & \textbf{49.08} & \textbf{34.02}  & \textbf{49.51} & \textbf{30.54}  & \textbf{47.27} \\
% \bottomrule
% \end{tabular}
% \end{table*}


% % \begin{table}[htbp]\small
% % \centering
% % \begin{center}
% % \caption{White-box Adversarial Robustness of MobileNet-V2 on CIFAR-10 and CIFAR-100 Datasets.}
% % \label{tab_eval_White_cifar10_cifar100_MobileNet-V2}
% % \vspace{-0.075in}
% % \setlength{\tabcolsep}{0.1mm}{
% % \begin{tabular}{c|c|ccc|ccc}
% % \toprule
% % \multirow{2}{*}{Attack} & \multirow{2}{*}{Defense} & \multicolumn{3}{c|}{CIFAR-10} & \multicolumn{3}{c}{CIFAR-100} \\
% %  &  & Clean & Robust & W-Robust & Clean & Robust & W-Robust \\
% % \midrule
% % \multirow{11}{*}{FGSM} 
% % & Natural    & 93.35  & 12.22  & 52.79                      & 75.18  & 7.96   & 41.57 \\
% % & SAT        & 83.87  & 55.89  & 69.88                      & 56.16  & 25.88  & 41.02 \\
% % & TRADES     & 77.95  & 53.75  & 65.85                      & 57.75  & 31.36  & 44.56 \\
% % & ARD        & 83.43  & 57.03  & 70.23                      & 60.11  & 33.61  & 46.86 \\
% % & RSLAD      & 83.20  & \textbf{59.47}  & 71.34                      & 58.25  & 34.73  & 46.49 \\
% % & SCORE      & 82.32  & 58.43  & 70.38                      & 58.25  & 34.73  & 46.49 \\
% % & Fair-ARD   & 82.65  & 56.37  & 69.51                      & 58.25  & 34.73  & 46.49 \\
% % & ABSLD      & 82.50  & 58.47  & 70.49                      & 58.25  & 34.73  & 46.49 \\
% % & MTARD      & \uline{89.26}  & 57.84  & 73.55                      & 64.30  & 31.49  & \cellcolor{gray!40}47.90  \\
% % & B-MTARD    & 89.09  & 58.79  & \uline{73.94}                      & 64.30  & 31.49  & \cellcolor{gray!40}47.90  \\
% % & CIARD      & \textbf{89.51}  & \uline{59.10}  & \textbf{74.31}             & 65.99  & 38.01  & \textbf{52.00} \\
% % \cmidrule{1-8}
% % \multirow{11}{*}{PGD$_\text{sat}$} 
% % & Natural    & 93.35  & 0      & 46.68                      & 75.18  & 7.96   & 41.57 \\
% % & SAT        & 83.87  & 46.84  & 65.36                      & 56.16  & 25.88  & 41.02 \\
% % & TRADES     & 77.95  & 49.06  & 63.51                      & 57.75  & 31.36  & 44.56 \\
% % & ARD        & 83.43  & 49.50  & 66.47                      & 60.11  & 33.61  & 46.86 \\
% % & RSLAD      & 83.20  & \uline{53.25}  & 68.23                     & 58.25  & 34.73  & 46.49 \\
% % & SCORE      & 82.32  & \textbf{53.42}  & 67.87                      & 58.25  & 34.73  & 46.49 \\
% % & Fair-ARD   & 82.65  & 50.50  & 66.58                      & 58.25  & 34.73  & 46.49 \\
% % & ABSLD      & 82.50  & 52.98  & 67.74                      & 58.25  & 34.73  & 46.49 \\
% % & MTARD      & \uline{89.26}  & 44.16  & 67.71                      & 64.30  & 31.49  & \cellcolor{gray!40}47.90  \\
% % & B-MTARD    & 89.09  & 47.56  & \uline{68.33}                      & 64.30  & 31.49  & \cellcolor{gray!40}47.90  \\
% % & CIARD      & \textbf{89.51}  & 47.67  & \textbf{68.59}             & 65.99  & 38.01  & \textbf{52.00} \\
% % \cmidrule{1-8}
% % \multirow{11}{*}{PGD$_\text{trades}$} 
% % & Natural    & 93.35  & 0      & 46.68                      & 75.18  & 7.96   & 41.57 \\
% % & SAT        & 83.87  & 49.14  & 66.51                      & 56.16  & 25.88  & 41.02 \\
% % & TRADES     & 77.95  & 50.27  & 64.11                      & 57.75  & 31.36  & 44.56 \\
% % & ARD        & 83.43  & 51.70  & 67.57                      & 60.11  & 33.61  & 46.86 \\
% % & RSLAD      & 83.20  & \textbf{54.76}  & 68.98                     & 58.25  & 34.73  & 46.49 \\
% % & SCORE      & 82.32  & 54.46  & 68.39                      & 58.25  & 34.73  & 46.49 \\
% % & Fair-ARD   & 82.65  & 52.12  & 67.39                      & 58.25  & 34.73  & 46.49 \\
% % & ABSLD      & 82.50  & \uline{54.49}  & 68.50                      & 58.25  & 34.73  & 46.49 \\
% % & MTARD      & \uline{89.26}  & 47.99  & 68.63                      & 64.30  & 31.49  & \cellcolor{gray!40}47.90  \\
% % & B-MTARD    & 89.09  & 50.44  & \uline{69.77}                      & 64.30  & 31.49  & \cellcolor{gray!40}47.90  \\
% % & CIARD      & \textbf{89.51}  & 50.71  & \textbf{70.11}             & 65.99  & 38.01  & \textbf{52.00} \\
% % \cmidrule{1-8}
% % \multirow{11}{*}{CW$_{\infty}$} 
% % & Natural    & 93.35  & 0      & 46.68                      & 75.18  & 7.96   & 41.57 \\
% % & SAT        & 83.87  & 46.62  & 65.25                      & 56.16  & 25.88  & 41.02 \\
% % & TRADES     & 77.95  & 46.06  & 62.01                      & 57.75  & 31.36  & 44.56 \\
% % & ARD        & 83.43  & 48.96  & 66.20                      & 60.11  & 33.61  & 46.86 \\
% % & RSLAD      & 83.20  & \textbf{51.78}  & 67.49                     & 58.25  & 34.73  & 46.49 \\
% % & SCORE      & 82.32  & 49.18  & 65.75                      & 58.25  & 34.73  & 46.49 \\
% % & Fair-ARD   & 82.65  & \uline{51.07}  & 66.86                      & 58.25  & 34.73  & 46.49 \\
% % & ABSLD      & 82.50  & 50.20  & 66.35                      & 58.25  & 34.73  & 46.49 \\
% % & MTARD      & \uline{89.26}  & 43.42  & 66.34                      & 64.30  & 31.49  & \cellcolor{gray!40}47.90  \\
% % & B-MTARD    & 89.09  & 46.81  & \uline{67.95}                      & 64.30  & 31.49  & \cellcolor{gray!40}47.90  \\
% % & CIARD      & \textbf{89.51}  & 46.88  & \textbf{68.20}             & 65.99  & 38.01  & \textbf{52.00} \\
% % \bottomrule
% % \end{tabular}
% % }
% % \vspace{-0.075in}
% % \end{center}
% % \end{table}


% \noindent\textbf{Black-box Robustness of Student Models.}
% We also performed black-box evaluations, incorporating both transfer-based and query-based~\cite{andriushchenko2020square} methods, to assess the student model's robustness in environments more akin to real-world scenarios. The parameter configurations for the student and teacher models were consistent with those used in the white-box evaluations. 

% Using CIFAR-10 and CIFAR-100, we evaluated the defensive capabilities of CIARD and other methods against black-box attacks on ResNet-18 and MobileNet-V2, focusing on both transfer-based and query-based attacks. For transfer-based attacks, we used adversarial teachers (WideResNet-34-10 and WideResNet-70-16) to generate adversarial examples for PGD$_\text{trades}$ and CW$_{\infty}$ attacks. For query-based attacks, we employed Square Attack (SA). We selected the best checkpoints for the baseline model and MTARD based on weighted robustness accuracy. Tables~\ref{tab_black_box_cifar10_cifar100_ResNet-18} and ~\ref{tab_black_box_cifar10_cifar100_MobileNet-V2} indicate that CIARD generally exhibits stronger resilience against the three types of black-box attacks. Notably, against PGD$_\text{trades}$ attacks, the student model achieved weighted robustness accuracy in CIFAR-10 that was 1.64\% and 0.66\% higher than the second-best methods, respectively. In summary, the experimental results clearly demonstrate the superior performance of CIARD in defending against both white-box and black-box attacks. Based on experimental results, ARD, RSLAD, MTARD, and CIARD outperform SAT and TRADES, demonstrating that ARD methods are more effective in enhancing small model performance compared to traditional approaches. 
% % Moreover, CIARD does not require manual hyperparameter tuning, yet it still surpasses ARD, RSLAD, and MTARD. In contrast, traditional methods like ARD and RSLAD require manual adjustments of the temperature constant % $\tau$ and loss weights. This raises an important question: Can analyzing and optimizing the hyperparameters within the teacher-student model framework further improve performance? We will explore this question in detail in the next experimental section.

% \begin{table}[htbp]\small
% \centering
% \begin{center}
% \caption{Black-box Adversarial Robustness of ResNet-18 on CIFAR-10 and CIFAR-100 Datasets.}
% \label{tab_black_box_cifar10_cifar100_ResNet-18}
% \vspace{-0.075in}
% \setlength{\tabcolsep}{0.1mm}{
% \begin{tabular}{c|c|ccc|ccc}
% \toprule
% \multirow{2}{*}{Attack} & \multirow{2}{*}{Defense} & \multicolumn{3}{c|}{CIFAR-10} & \multicolumn{3}{c}{CIFAR-100} \\
%  &  & Clean & Robust & W-Robust & Clean & Robust & W-Robust \\
% \midrule
% \multirow{10}{*}{PGD$_\text{trades}$} 
% & SAT        & 84.20  & 64.74  & 74.52                     & 56.16  & 38.10  & 47.13 \\
% & TRADES     & 83.00  & 63.61  & 73.31                     & 57.75  & 38.20  & 47.98 \\
% & ARD        & 84.11  & 63.50  & 73.81                     & 60.11  & 39.53  & 49.82 \\
% & RSLAD      & 83.99  & 63.96  & 73.98                     & 58.25  & 39.93  & 49.09 \\
% & SCORE      & 84.43  & 64.34  & 74.39                     & 58.25  & 39.93  & 49.09 \\
% & Fair-ARD   & 83.41  & 63.31  & 73.36                     & 58.25  & 39.93  & 49.09 \\
% & ABSLD      & 83.21  & 62.91  & 73.06                     & 58.25  & 39.93  & 49.09 \\
% & MTARD      & 87.36  & 65.26  & 76.31                     & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & B-MTARD    & \uline{88.20}  & \uline{65.29}  & \uline{76.75}    & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & CIARD      & \textbf{88.69}  & \textbf{66.07}  & \textbf{77.38}            & 65.99  & 42.21  & \textbf{54.10} \\
% \cmidrule{1-8}
% \multirow{10}{*}{CW$_{\infty}$} 
% & SAT        & 84.20  & 63.84  & 74.02                     & 56.16  & 38.10  & 47.13 \\
% & TRADES     & 83.00  & 62.83  & 72.92                     & 57.75  & 38.20  & 47.98 \\
% & ARD        & 84.11  & 62.86  & 73.49                     & 60.11  & 39.53  & 49.82 \\
% & RSLAD      & 83.99  & 63.05  & 73.52                     & 58.25  & 39.93  & 49.09 \\
% & SCORE      & 84.43  & 63.79  & 74.11                     & 58.25  & 39.93  & 49.09 \\
% & Fair-ARD   & 83.41  & 62.76  & 73.09                     & 58.25  & 39.93  & 49.09 \\
% & ABSLD      & 83.21  & 62.19  & 72.70                     & 58.25  & 39.93  & 49.09 \\
% & MTARD      & 87.36  & 64.58  & 75.97                     & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & B-MTARD    & \uline{88.20}  & \uline{64.64}  & \uline{76.42}    & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & CIARD      & \textbf{88.69}  & \textbf{64.79}  & \textbf{76.74}            & 65.99  & 42.21  & \textbf{54.10} \\
% \cmidrule{1-8}
% \multirow{10}{*}{SA~\cite{andriushchenko2020square}} 
% & SAT        & 84.20  & 72.48  & 78.34                     & 56.16  & 38.10  & 47.13 \\
% & TRADES     & 83.00  & 72.49  & 77.75                     & 57.75  & 38.20  & 47.98 \\
% & ARD        & 84.11  & 74.60  & 79.36                     & 60.11  & 39.53  & 49.82 \\
% & RSLAD      & 83.99  & 72.47  & 78.23                     & 58.25  & 39.93  & 49.09 \\
% & SCORE      & 84.43  & 74.68  & 79.56                     & 58.25  & 39.93  & 49.09 \\
% & Fair-ARD   & 83.41  & 74.08  & 78.75                     & 58.25  & 39.93  & 49.09 \\
% & ABSLD      & 83.21  & 73.93  & 78.57                     & 58.25  & 39.93  & 49.09 \\
% & MTARD      & 87.36  & 78.58  & 82.97                     & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & B-MTARD    & \uline{88.20}  & \uline{79.82}  & \uline{84.01}    & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & CIARD      & \textbf{88.69} & \textbf{79.91}  & \textbf{84.30}            & 65.99  & 42.21  & \textbf{54.10} \\
% \cmidrule{1-8}
% \end{tabular}
% }
% \vspace{-0.075in}
% \end{center}
% \end{table}


% \begin{table}[htbp]\small
% \centering
% \begin{center}
% \caption{Black-box Adversarial Robustness of MobileNet-V2 on CIFAR-10 and CIFAR-100 Datasets.}
% \label{tab_black_box_cifar10_cifar100_MobileNet-V2}
% \vspace{-0.075in}
% \setlength{\tabcolsep}{0.1mm}{
% \begin{tabular}{c|c|ccc|ccc}
% \toprule
% \multirow{2}{*}{Attack} & \multirow{2}{*}{Defense} & \multicolumn{3}{c|}{CIFAR-10} & \multicolumn{3}{c}{CIFAR-100} \\
%  &  & Clean & Robust & W-Robust & Clean & Robust & W-Robust \\
% \midrule
% \multirow{10}{*}{PGD$_\text{trades}$} 
% & SAT        & 83.87  & 64.66  & 74.27                     & 56.16  & 38.10  & 47.13 \\
% & TRADES     & 77.95  & 61.04  & 69.50                     & 57.75  & 38.20  & 47.98 \\
% & ARD        & 83.43  & 63.28  & 73.36                     & 60.11  & 39.53  & 49.82 \\
% & RSLAD      & 83.20  & 64.33  & 73.77                     & 58.25  & 39.93  & 49.09 \\
% & SCORE      & 82.32  & 63.84  & 73.08                     & 58.25  & 39.93  & 49.09 \\
% & Fair-ARD   & 82.65  & 62.62  & 72.64                     & 58.25  & 39.93  & 49.09 \\
% & ABSLD      & 82.50  & 62.91  & 72.71                     & 58.25  & 39.93  & 49.09 \\
% & MTARD      & \uline{89.26}  & 66.30  & 77.78                     & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & B-MTARD    & 89.09  & \uline{66.47}  & \uline{77.78}    & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & CIARD      & \textbf{89.51} & \textbf{66.66}  & \textbf{78.09}            & 65.99  & 42.21  & \textbf{54.10} \\
% \cmidrule{1-8}
% \multirow{10}{*}{CW$_{\infty}$} 
% & SAT        & 83.87  & 64.24  & 74.06                     & 56.16  & 38.10  & 47.13 \\
% & TRADES     & 77.95  & 60.66  & 69.31                     & 57.75  & 38.20  & 47.98 \\
% & ARD        & 83.43  & 62.83  & 73.13                     & 60.11  & 39.53  & 49.82 \\
% & RSLAD      & 83.20  & 63.45  & 73.33                     & 58.25  & 39.93  & 49.09 \\
% & SCORE      & 82.32  & 63.03  & 72.68                     & 58.25  & 39.93  & 49.09 \\
% & Fair-ARD   & 82.65  & 62.00  & 72.32                     & 58.25  & 39.93  & 49.09 \\
% & ABSLD      & 82.50  & 61.87  & 72.19                     & 58.25  & 39.93  & 49.09 \\
% & MTARD      & \uline{89.26}  & 65.68  & 77.47                     & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & B-MTARD    & 89.09  & \uline{65.96}  & \uline{77.53}    & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & CIARD      & \textbf{89.51} & \textbf{66.12}  & \textbf{77.82}            & 65.99  & 42.21  & \textbf{54.10} \\
% \cmidrule{1-8}
% \multirow{10}{*}{SA~\cite{andriushchenko2020square}} 
% & SAT        & 83.87  & 73.01  & 78.44                     & 56.16  & 38.10  & 47.13 \\
% & TRADES     & 77.95  & 67.43  & 62.69                     & 57.75  & 38.20  & 47.98 \\
% & ARD        & 83.43  & 73.26  & 78.35                     & 60.11  & 39.53  & 49.82 \\
% & RSLAD      & 83.20  & 73.07  & 78.14                     & 58.25  & 39.93  & 49.09 \\
% & SCORE      & 82.32  & 72.41  & 77.37                     & 58.25  & 39.93  & 49.09 \\
% & Fair-ARD   & 82.65  & 72.44  & 77.55                     & 58.25  & 39.93  & 49.09 \\
% & ABSLD      & 82.50  & 72.05  & 77.28                     & 58.25  & 39.93  & 49.09 \\
% & MTARD      & \uline{89.26}  & 79.13  & 84.20                     & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & B-MTARD    & 89.09  & \uline{79.61}  & \uline{84.35}    & 64.30  & 41.39  & \cellcolor{gray!40}52.85  \\
% & CIARD      & \textbf{89.51} & \textbf{80.01}  & \textbf{84.76}            & 65.99  & 42.21  & \textbf{54.10} \\
% \cmidrule{1-8}
% \end{tabular}
% }
% \vspace{-0.075in}
% \end{center}
% \end{table}
